VBridge: Connecting the Dots Between Features and Data to Explain Healthcare Models

Machine learning (ML) is increasingly applied to Electronic Health Records (EHRs) to solve clinical prediction tasks. Although many ML models perform promisingly, issues with model transparency and interpretability limit their adoption in clinical practice. Directly using existing explainable ML techniques in clinical settings can be challenging. Through literature surveys and collaborations with six clinicians with an average of 17 years of clinical experience, we identified three key challenges, including clinicians' unfamiliarity with ML features, lack of contextual information, and the need for cohort-level evidence. Following an iterative design process, we further designed and developed VBridge, a visual analytics tool that seamlessly incorporates ML explanations into clinicians' decision-making workflow. The system includes a novel hierarchical display of contribution-based feature explanations and enriched interactions that connect the dots between ML features, explanations, and data. We demonstrated the effectiveness of VBridge through two case studies and expert interviews with four clinicians, showing that visually associating model explanations with patients' situational records can help clinicians better interpret and use model predictions when making clinician decisions. We further derived a list of design implications for developing future explainable ML tools to support clinical decision-making.

==> README <==
Created by Torsten Moeller (vis@cs.sfu.ca), April 6 2004
modified by Steven Bergner and Torsten Moeller, June 30 2006
modified by James Peltier and Torsten Moeller, March 28, 2007
modified by Bernhard Finkbeiner, July 5, 2010
modified by Tobias Isenberg, January 2016
modified by Filip Sadlo, March 2016
modified by Tobias Isenberg, July 2016

This distribution provides a document class for formatting papers according to the specifications for submission to conferences sponsored by the IEEE Visualization & Graphics Technical Committee (VGTC).

Conferences that use the 'journal' document option:
- IEEE Visualization Conference (VIS, incl. InfoVis, SciVis, VAST)
- IEEE Virtual Reality (VR)
- IEEE International Symposium on Mixed and Augmented Reality (ISMAR)

It contains 13 files/directories:

README          - this file
diamondrule.eps - abstract and body separator
diamondrule.pdf - its PDF version
vgtc.cls        - the VGTC class file, which should be placed, somewhere in the TeX search path (or in the local directory)
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
template.pdf    - an example proper pdf output in default journal mode
abbrv-doi*.bst  - four different versions to generate the bibliography including DOI output, with and without hyperref support, with and without narrow rendering of DOIs
makefile        - makefile including bibtex compilation and proper PDF generation
pictures/       - subdirectory with sample images, both in EPS and in direct pixel/vector format

Usage
=====

The template can be used as such (using the established LaTeX environments) by calling pdfLaTeX or LaTex. For Windows-based LaTeX installations you can use, for example, the environment provided by http://www.texniccenter.org/ along with MikTeX (http://miktex.org/). For Uinux-based installations, please use your favorite LaTeX distribution and editing environment or use the makefile following the instructions below.

Use of the Makefile
===================

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create a file called 'template.pdf'. Please make sure, that its layout is identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process manually.  Below are a list of available options that may be passed to make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> content/_backup-related-work-Mar8.tex <==
\section{Related Work}

% \fan{Make sure to address what is special about ``explainable predictive models for healthcare'' vs. ``other explainable predictive models'' (e.g., VAST best paper 2020 about XAI for self-driving cars)}
% characteristics of medical records: high dimensionality, irregularity in time, and sparsity.

EHRs contain a wealth of high-dimensional heterogeneous data from structured attributes (\eg, demographic information, diagnoses, and medications) to unstructured ones (\eg, clinical notes and medical images).
Our focus is structured attributes and following we will discuss the most relevant work.

\subsection{Explainable Machine Learning on Clinical Predictions}
% Surveys: \cite{payrovnaziri2020explainable} \cite{tjoa2020survey}
% Evaluations: \cite{wang2019designing} \cite{tonekaboni2019clinicians}

% In the healthcare field, the interpretability of ML prediction models is paramount due to the factors including risk and responsibilities that other fields may not consider.
Two recent surveys~\cite{payrovnaziri2020explainable, tjoa2020survey} have systematically reported the current progress of existing XAI techniques for clinical use.
Among these techniques, we focus on the ones that provide local explanations -- the explanations for understanding why the model make a certain prediction for a patient.
Following a widely accepted taxonomy~\cite{molnar2020interpretable}, we further categorize these techniques based on whether the provided interpretability is intrinsic or post-hoc.

\textbf{Intrinsic interpretability.}  \label{sec:related:xai_intrinsic}
Models incorporating interpretability directly to their structures provide intrinsic interpretability.
The models of this category are often of less-complex structures to allow for accurate and faithful explanations.
Examples include decision tree~\cite{kho2012use} which identifies a set of rules to predict genetic risk for type 2 diabetes, k-nearest neighbors~\cite{gallego2015bringing} which finds similar patients for support bedside clinical decision-making, and linear model~\cite{fleisher2007clinical} which exposes a list of risk factors of progression to Alzheimer disease.
However, compared with complex ML models (\eg, deep neural networks), the performance of these models is bounded, especially when handling complex clinical prediction tasks~\cite{harutyunyan2019multitask, xiao2018opportunities}.
While boosting and optimization techniques can be used to enhance model performance, such as ensemble learning~\cite{jalali2016interpretable}, they introduce additional challenges to interpret the results as well.

Recent focuses have been put on to the attention-based neural networks ~\cite{payrovnaziri2020explainable, xiao_opportunities_2018}.
The attention mechanism does not inform clinicians of the direct answer of a prediction result but highlights the part of historical information (\eg, clinical events) which weighs more in predicting disease onsets to support decision-making~\cite{choi2016retain, kwon2018retainvis}.
Despite that deep learning models can produce accurate predictions, attention-based explanations may cause information overload and confuse clinicians due to the lack of clarity on how the prediction results are related to the areas of attention~\cite{payrovnaziri2020explainable}.
Another drawback is that it is challenging for attention-based deep learning models to support multimodal learning while still preserve good interpretability~\cite{xiao_opportunities_2018}.
Our scenario, however, requires to use patient's multimodal data from demographics information, prescriptions, lab test results and continuous monitoring data during ICU, to predict the risk of post-surgery complications.
% Though multitask learning method which jointly learns data across multiple modalities can be used, .. 

\textbf{Post-hoc interpretability}.  \label{sec:related:xai_posthoc}
Post-hoc methods take the ``black-box'' ML models as inputs and derive explanations for model predictions. The underlying model performance remains intact.
One common approach is to use an intrinsically interpretable ML model of less complexity to mimic the target ``black-box'' ML model. 
For example, Che \etal\ \cite{che2016interpretable} worked on acute lung injury (ALI) prediction and proposed a knowledge distillation method called mimic-learning, using gradient boosting trees to mimic the original deep learning model and provide rule explanations to clinicians. 
% Ming \etal\ \cite{ming2018rulematrix} used Baysian Rule List~\cite{letham2015interpretable} to surrogate the target model built for breast cancer diagnosis and diabetes classification and further visualize the rule list for better result interpretation.

Another type of work focuses on calculating feature importance, which is considered as one of the top approaches (the other one is attention mechanism) supporting local explanations~\cite{payrovnaziri2020explainable}.
Ribeiro \etal ~\cite{ribeiro2016should} proposed the local interpretable model-agnostic explanation (LIME), which perturbs an instance, generates neighborhood samples, and learns an local interpretable model to explain the prediction of the instance.
Pan \etal ~\cite{pan2019development} and Ghafouri-Fard~\cite{ghafouri2019application} leveraged LIME to derive the contributions of features for the tasks of predicting girl's central precocious puberty and autism spectrum disorder respectively.
Lundberg \etal\ introduced Shapley Additive Explanations (SHAP)~\cite{NIPS2017_7062}, a game-theoretic approach to calculate the contributions of each feature to the predictions. SHAP and its extensions~\cite{lundberg2020local} has been used to support clinical decisions, for example, explaining in-surgery hypoxaemia predictions for early prevention~\cite{lundberg2018explainable}. 

In this work, we aim to solve the three practical challenges (refer to Sec.~\ref{sec:intro}) facing deploying feature-importance-based XAI techniques for supporting clinical decision-making. %Specially, xxx algorithm.


\subsection{Electronic Health Records Visualization}
Visualization techniques have been extensively used to analyze EHR data for knowledge discovery~\cite{Rind2013Survey, west2015innovative, Jin2020CarePre}.
We classify the existing visualization techniques based on the criterion proposed by Rind \etal ~\cite{Rind2013Survey} -- whether they are designed for the exploration and querying of health records from one individual patient or multiple patients.   
% Many visual analysis systems have been developed for representing and analyzing electronic health records~\cite{Jin2020CarePre}.
% A comprehensive survey of electronic health record visualizations by Rind \etal ~\cite{Rind2013Survey} states that the number of patient records used is a strongly differentiating criterion for taxonomy, i.e., individual or multiple patient records used in the visual analysis system.

\textbf{Individual patient records.} 
The goal of visualizing individual patient records is to provide individual patient summaries as well as an efficient way to explore personal complex record data at different level of detail.
A patient's clinical records contain longitudinal data of patient visits over time.
% provide patient summary
To summarize such history, one common way is to use timeline-based visualization, where events are placed on a horizontal timeline chronologically using points or interval plots~\cite{Plaisant1998Lifelines, Shahar1999KNAVEI, Shahar2006KNAVEII}.
% multiple types of events: hierarchical
Multiple stacked rows with hierarchical structures may be used when there is a need to distinguish different event types~\cite{Plaisant1998Lifelines}. 
% multiple attributes of an event: table (flowsheet) && glyph 
However, an individual event (\eg, lab test) may consist of multiple attributes.
To depict this information, one popular approach is providing an interactive table which shows key clinical variables from one or multiple events over a period of time~\cite{bauer2006evaluating, Ghassemi2018ClinicalVis}.
The other common approach is using glyphs to encode multivariate events~\cite{Zhang2019IDMVis}. 


% solve scalability issue with simplification
Noticing the need to scale to huge numbers of event types and handle complex event attributes, recent work has switched the focus to visualize patterns instead of depicting every event in detail. Researchers have explored aggregation-based  methods~\cite{krstajic2011cloudlines} and substitution-based approaches~\cite{Gotz2014DecisionFlow} to address different analytical needs.
% query, pattern search, and filtering
Another line of research is developing methods for event pattern searching, filtering, and grouping~\cite{wongsuphasawat2009finding, wongsuphasawat2012querying} to support efficient data exploration.

% Early visualization systems focus on analyzing a single record~\cite{Plaisant1998Lifelines, Shahar1999KNAVEI, Shahar2006KNAVEII, Gotz2014DecisionFlow, Zhang2019IDMVis, Li2020DGViz}.
% The most common visualization is to use timeline-based representation, since a patient record is often regarded as time event sequence~\cite{Gotz2014DecisionFlow}.
% Events are placed on a horizontal timeline chronologically using point or interval plots.
% The records of one individual patient may consist of multiple stacked rows, each plotting one type of events and organized by facets or categories as a comprehensible hierarchical structures~\cite{Plaisant1998Lifelines}.
% Expect juxtaposition, IDMVis superimposes distinct visualizations of all needed multivariate data (CGM readings, blood glucose level, logbook events) in a single row for one day, and combines 14-day records with small multiples and event alignment to better show records for a single diabetes patient ~\cite{Zhang2019IDMVis}.
% The events are usually encoded to different representations, like icons with different shapes and different colors or glyphs.

Clinical signals collected during ICU or surgery are also a common type of EHR data. Our model uses this information to predict post-surgery complications. 
This type of data is usually sampled at a higher frequency and can be viewed as time series data.
Numerous methods for visualizing time series data~\cite{aigner2011visualization} can be utilized.
For example, line plot with horizontal timeline is used to visualize patient's vital signs in ICU~\cite{levy-lambert2018visualizingICU}. Xu \etal~\cite{Xu2018ECGLens} leverage spiral timeline to reveal periodic patterns of electrocardiogram data for arrhythmia detection.

% While for those time series data, like vital signs during surgery, they are usually represented by line plots and also organized along a timeline, however, not only the trivial horizontal ones ~\cite{levy-lambert2018visualizingICU, Vong2016IVA}, but also the spiral ones to reveal periodic patterns in time series~\cite{Xu2018ECGLens}.
% What's more, some work use annotations to identify the important components to help clinicians get the significant information from large-scale data and make decision efficiently~\cite{Xu2018ECGLens}.

% Specifically, sometimes the timeline visualization is just show the occurrence of the events without detailed values, and the hovering capabilities with popup windows with details is provided. 
% Also, providing a table shows the detailed values with aggregated events on specific time is another intuitive method~\cite{Ghassemi2018ClinicalVis}.
% The Flowsheet, a combination of spreadsheets, time, and detailed value or presentation of the data, is regarded as the most widely used interface by nurses and physicians to get a quick overview of the patient’s condition~\cite{Reddy2001Coordinating, Rind2013Survey}. 
% The columns is aligned with the horizontal timeline, while the cells in each row is number or marks in point or interval.
% While the unstructured data like notes and images are usually represented as text description and raw images.


In practice, given the truth of heterogeneity of EHR data, many visualization systems have adopted multiple coordinated views with each view displaying a certain type of information using the aforementioned techniques.
\system~ uses the same strategy and leverages many of the advances offered by prior visualization techniques.
Notably, the core goal of our system is to provide local explanations to clinicians, which differentiates our system from the prior visualization systems substantially.
In this regard, we propose a novel visualization to show feature importance in a hierarchical and scalable manner and then visually connecting these explanations back to patients' original records.
% In real application, most systems will consider heterogeneous data rather than just one data type. Thus, different visualizations may be composited together by multiple views or integration.


\textbf{Multiple patient records.}
There are many scenarios requiring multiple patient records analysis~\cite{Rind2013Survey} ranging from monitoring patient cohorts and patient alarm specification to clinical trial recruitment and observational clinical research.
A system supporting the analysis of patient record collections focuses more on finding high-level patterns common to a number of patients.
To represent multiple patient records, one typical approach is to composite each individual patient records using small multiples~\cite{kwon2018retainvis, Jin2020CarePre}.
Though effective, these techniques are difficult to scale up to large numbers of patients.
To improve scalability, researchers have explored many flow-based representations to highlight the frequent patterns of clinical event sequences.
OutFlow~\cite{wongsuphasawat2011outflow} aggregates multiple event sequences based on a graph-based model and LifeFlow~\cite{Wongsuphasawat2011LifeFlow} summarizes multiple event sequences using a tree structure.
DecisionFlow~\cite{Gotz2014DecisionFlow} further improves the scalability by visualizing large numbers of event types based on several key events.

Rather than showing frequent patterns, one of the key focuses of this work is to provide evidence (\eg, reference values) from a cohort of patients of interest to help clinicians assess feature importance values offered by our XAI algorithm. One close work is done by Stubbs \etal~\cite{2012SimTwentyFive} which uses transparent band superimposed on patient ICU time series data to reveal the $mean \pm SD$ of the similar patient group to facilitate clinicians better understanding of the data.
However, our scenario is much more complex and challenging; we have to consider aligning the reference values (\ie, aggregated values) with not only the feature-level explanations but also the heterogeneous patient records including demographics information, diagnoses results, clinical events, and ICU time series.


%%% **************** Obsolete Versions **************** %%%

%%%-----------------XAI in Clinical-------------------
% % Explainable machine learning techniques have been increasingly proposed and adopted to support clinical decision-makings~\cite{payrovnaziri2020explainable}. 
% Explainable machine learning techniques have been increasingly proposed to support clinical decision-makings~\cite{payrovnaziri2020explainable}.
% The progress of the approaches have been summarized in recent surveys~\cite{tjoa2020survey, payrovnaziri2020explainable}. 
% We adopt a widely accepted taxonomy to organize this section, where existing works are categorized into intrinsically interpretable models and post-hoc methods.

% % Intrinsically interpretable models  
% % Existing works:
% % attention-based~\cite{choi2016retain, shickel2019deepsofa, Jin2020CarePre, kwon2018retainvis, li2020marrying}, 
% % generative additive model(GAM)~\cite{lou2012intelligible, lou2013accurate, caruana2015intelligible}, 
% % rule-based~\cite{letham2015interpretable}

% \textbf{Intrinsically interpretable models.} 
% Building both accurate and interpretable machine learning models is always desired by the AI community.
% Traditional ML models, like logistic regression, decision tree, are interpretable due to their simple model structures. However, their performance in complex clinical prediction tasks is very limited~\cite{harutyunyan2019multitask}. 
% To make better trade-offs between accuracy and interpretability, Lou \etal\ proposed GA\textsuperscript{2}Ms~\cite{lou2013accurate} extended from Generalized Additive Models (GAMs)~\cite{lou2012intelligible}. 
% The following work by Caruana \etal\ uses GA\textsuperscript{2}Ms to predict patients' pneumonia risk and hospital readmission and explain the predictions with partial dependency plots (PDPs). 
% Other interpretable models, like decision list~\cite{letham2015interpretable} and decision set~\cite{lakkaraju2016interpretable}, use a set of IF-THEN rules to form the models' decision paths. 

% Recent focuses have been put on to the attention mechanism~\cite{vaswani2017attention, choi2016retain, shickel2019deepsofa, Jin2020CarePre, kwon2018retainvis, li2020marrying}.
% Choi \etal\ proposed Retain~\cite{choi2016retain}, an attention-based interpretable model that takes patients' longitudinal records to make predictions. The attention weights can be used to find the highly influential features to the prediction results. Kwon \etal\ extent the Retain model and built RetainVis~\cite{kwon2018retainvis} to support interactive model explorations. 



% \textbf{Post-hoc interpretability}.
% Post-hoc methods take the ``black-box'' ML models as inputs and derive explanations for model predictions.
% One common approach is to use an interpretable ML model to mimic the target ``black-box'' ML model. 
% Che \etal\ worked on acute lung injury (ALI) prediction and proposed a knowledge distillation method called mimic-learning~\cite{che2016interpretable}, using gradient boosting trees to mimic the original deep learning model and provide rule explanations to clinicians. 
% Ming \etal\ followed a similar idea of using Baysian Rule List~\cite{letham2015interpretable} to surrogate the target model and designed a scalable visualization~\cite{ming2018rulematrix} to filter and inspect the rules. 
% Another type of works focuses on calculating and presenting feature interactions and importance. 
% Lundberg \etal\ introduced Shapley Additive Explanations (SHAP)~\cite{NIPS2017_7062}, a game-theoretic approach to calculate the contributions of each feature to the predictions. SHAP and its extensions~\cite{lundberg2020local} has been used to support clinical decisions, for example, explaining in-surgery hypoxaemia predictions for early prevention~\cite{lundberg2018explainable}. 

% Despite of the success of existing works in opening the ``block-box'' machine learning models, they stop on making explanations with artificial features, remaining a gap from the current medical practice, \ie, making decisions from patients' original records. 
% In our work, we investigate the clinicians' need in incorporating feature-level explanations with their current workflow and present [System Name] to fill this gap.

% Li. etc transform MIMIC-II dataset to a tabular dataset containing 8 features, and show the different contributions of these features on different ML models on a specific prediction task, i.e., predicting in-hospital mortality, to assist clinicians to understand, compare and evaluate the model performance intuitively~\cite{LI2020122}.


%%%-----------------EHR Vis -----------------

% V1 - single patient
% Scenarios that just require working with a single patient record include providing an overview of the patient history to understand trends[cite:dashboard, diabates], identify significant events[cite: XuECG], spot omissions in data or treatment and etc to support core clinical care tasks.
% A patient’s EHR data contain information of a patient’s visits over time. 
% It is usually recorded as a sequence of medical codes, where each code corresponds to either a doctor’s diagnosis of a patient, a treatment or surgery, medical or lab test event, or a prescriptions.
% Thus, EHR visualization is often closely aligned with the problems of temporal event sequence visualization.
% In this case, researchers tend to encode these discrete events or medical codes to different representations, like icons with different shapes and different colors or glyphs, and display them using common axes considering real time gap or just using equal distance [cite: Lifelines, IDMVis, DG-Viz, KNAVE I and II].
% For example, Lifelines encodes normal or abnormal status of multiple medical events with different color and show them by point or interval plot along time.
% Inspired by Lifeline, IDMVis superimposes distinct visualizations of multivariate data (CGM readings, blood glucose level, logbook events) combined with small multiples and sentinel event alignment to better show a single diabetes patient records for 14 days.

% Besides the discrete data, the EHR data also contains continuous data, such as vital signs during surgery.
% For these continuous data, some researchers tend to use statistical value to summarize the whole time series[cite:].
% While some work show the raw time series data and identify the important components to help clinicians get the significant information from large-scale data and make decision efficiently [cite: Xu2018ECGLens].


% V1 - multiple patients
% Differing from single patient systems, the system supporting patient record collections emphasizes more on querying, defining similarity, comparing, aggregating, and clustering~\cite{Wang2009Lifelines2, MonroeEventFlow, Klimov2010VISITORS, Gotz2014DecisionFlow, Fan2017PeerFinder, kwon2018retainvis, Wentzel2020TSSIM, Jin2020CarePre} 
% [cite:EventFlow, LikeMeDonuts].
% To represent the multiple patient records, a common technique is to composite each individual patient records for the whole cohorts by different methods, e.g., juxtaposition~\cite{Wang2009Lifelines2, kwon2018retainvis, Jin2020CarePre}, and superimposition~\cite{Wentzel2020TSSIM},
% while some researchers provide novel measures to aggregate, often using flow-based techniques reminiscent of Sankey diagrams or a tree of sequence~\cite{Wongsuphasawat2011LifeFlow, Gotz2014DecisionFlow,  Fan2016EventAction, Guo2019ET2, Jin2020CarePre}[cite: Outflow, EventFlow].
% For example, LifeFlow summarizes multiple event sequences as a tree structure ~\cite{Wongsuphasawat2011LifeFlow}, while OutFlow aggregates multiple event sequences based on a graph-based model. 
% What's more, some works may aggregate the statistical value of selected patient group with the record of one specific patient to identify the location of this patient among the whole.
% For example, Stubbs et al. use area superimposed the patient raw data to represent the $mean \pm SD$ of the similar patient group to help clinicians better understand the data~\cite{2012SimTwentyFive}.

% Inspired by these work, we show both the individual patient records using point, interval, line plot, and also table records along timeline, and identify the location of the specific patient among the selected patient cohorts by the distribution plot and the superimposed area plot of $mean \pm SD$.

% Detailed description of some related work - Yanna
% Outflow captured all permutations of event occurrence based on a graph-based model. EventAction summarized event data occurring within a common time period, and explored potential outcomes for behavior prediction and recommendation.
% These techniques help communicate various forms of sequential patterns, but rely on permutations in the order of event type occurrence to build the visual representations.
% For example, EventFlow and DecisionFlow highlight the key events and summarize the medical records of patient group to reduce visual complexity,
% while CarePre provide a novel flow-based visualization to aggregate medical event sequence for the similar patients to illustrate the overall evolution of diseases and treatments over time~\cite{Jin2020CarePre}. 
% Also, since there are more than one patient records, some research provide the alignment technique to help users identify precursor, co-occurring, and aftereffect events[cite: Lifeline2].
% For example, Lifeline2 enables users to align all records by a specific clinical event, like heart attacks, then every record’s first heart attack event will then be aligned vertically.

==> content/_backup_introduction_v2.tex <==
\section{Introduction}

%%%------------------------- Background: ML for health care--------------------
Various prediction models based on machine learning (ML) techniques  have emerged over the rapid proliferation of Electronic Health Record (EHR) data to improve the quality of clinical care~\cite{solares2020deep, rajkomar2019machine}. 
EHR data records each individual's health journey from structured records, like demographic information, diagnoses, and medications, to unstructured ones, including clinical notes and medical images.
A prediction model takes one patient's historical records to predict the future health states, such as \textit{in-hospital mortality~\cite{harutyunyan2019multitask}}, \textit{remaining length of stay~\cite{rajkomar2018scalable}}, and \textit{post-surgery complications~\cite{}}.

% Not sure whether we should directly introduce our target problem and the type of data (static info plus temporal observation data, excluding unstructured data) we used here after we introduce the typical prediction problems.

%%%----------------- Background: Interpretability & Transparency-----------------

%%% V3
Despite the endeavour ML researchers have spent to improve model performance, the associated issues regarding transparency and interpretability that comes from real-world deployment process still remain challenging, especially in a highly regulated and risk-averse industry like healthcare~\cite{sendak2020human, payrovnaziri2020explainable}.
There are many XAI (eXplainable artificial intelligence) techniques/tools that have been developed and shown their power in opening the black-box of ML models. \hl{[XAI technique cases]} Nevertheless, prediction models built upon modern ML techniques yet have not been widely and reliably used in clinical decision support workflows~\cite{jensen2012mining, miotto2016deep, rajkomar2019machine}. 
Working with clinicians to solve a post-surgery cardiac complication prediction problem, we found that the gaps facing the introduction of XAI techniques into healthcare settings are twofold.

On the one hand, clinicians are frequently presumed to be equipped with sufficient technical expertise with which to engage with XAI tools to understand, debug, and even improve ML models~\cite{ahmad2018interpretable}. Concerns may arise when clinicians desire XAI tools to be more patient-oriented rather than technology-oriented. 
Moreover, in healthcare, clinicians are rarely involved in the discussions of explainability during the development of XAI tools~\cite{lipton2017doctor}. As a results, the potential solutions coming out eventually are intrinsically technical -- the explanations offered are more from the ML researchers' intuition of what constitutes a `good` explanation rather than practitioners~\cite{tonekaboni2019clinicians}. \hl{[case]}
% Hence, we may ask what auxiliary information alongside ML predictions is needed to facilitate the clinicians' interpreting of the results?

On the other hand, clinicians often work with individual patients and demand specific explanations tailored to each patient's health records (i.e., local explanations).
%for raising awareness of conditions or handling potential disagreements. 
Among copious XAI approaches supporting local explanations, feature importance is considered as one of the topmost. It illustrates the degree of contribution of the ML-input features to the prediction outcome~\cite{payrovnaziri2020explainable}. Knowing this, clinicians are able to compare model decision with their clinical judgement leveraging the domain experience, especially when there is a disagreement.
However, feature importance approaches, though extensively studied in XAI field, are still facing several significant challenges when it comes to actual use in healthcare.

%%%------------------- Challenges --------------------------

\begin{itemize}
    \item \textbf{Understand ML features.} 
    Not every feature inputted to ML models is easy to understand by clinicians because of the unfamiliarity of the data representation. For example, the linear slope of the patient's systolic blood pressure in the last 24 hours \hl{[glyph]}.
    Directly showing importance of such features is unhelpful for clinicians to gain deep insights.
    
    \item \textbf{Connect to patients' original records.}
    Clinicians are more familiar with patient's original records and usually make decisions referring to raw data such as laboratory test reports and vital signs from a caring machine. Existing XAI techniques of feature importance generate explanations in the space of ML features. How to connect these explanations back to patients' original records remained unexplored. 
    
    \item \textbf{Align with evidence.}
    Simply presenting a list of numerical values (feature contributions) to clinicians is insufficient for clinicians to incorporate their domain experience for model decision assessment. Enough contextual information regarding a certain patient should be provided~\cite{wang2019designing}, even ML models did not use those data such as clinical notes. More importantly, clinicians identified a need of explaining feature importance aligning with evidence-based medical practice~\cite{tonekaboni2019clinicians}. For example, \hl{example}.
\end{itemize}






%%%-------------------Method: Iterative Design Study--------------------------
%This work aims to integrate existing post-hoc explainability methods into clinicians' decision workflow by bridging the feature-level explanations with patients' original records with interactive visualization. 
The aforementioned challenges drove us to the development of a visual analytics solution to integrate feature-level explanations into clinicians' decision support workflow.
We followed a user-centric design process~\cite{wang2019designing,yang2019unremarkable} by working with clinicians from a children hospital since the start of developing our XAI tool.
We use Paediatric Intensive Care (PIC) Database\footnote{PIC is supplement to the well-known MIMIC database.} as our target dataset; it comprises information relating to young patients -- children under 18 years -- who are admitted to intensive care units (ICU).
% Compared with general patients, ICU patients have more data available such as the surgery information and the vital signals during surgery (viewed as multivariate time series).
% It is a supplement to MIMIC database, a well-known EHR dataset widly used in the research community. PIC dataset comprises information relating to patients (children younger than 18 years) 
% Our task is to predict the risk of cardiac complications after cardiac surgery, based on the patient's demographic information, surgery information, vital signs during surgery (i.e., multivariate time series), medications, and more.
% The dataset contains each patient's demographic information, surgery information, vital signs (time series) during surgery, etc.
% \furui{}{The lessons learned from the co-design process include: 1) }

%%%---------------Method: System/Techniques -----------------------
We presented a xxx workflow xxx.
Built upon the workflow, we designed and developed NAME, an interactive visualization system, to facilitate clinicians' understanding and interpreting the predictions of ML models.
The system (what technique has been used? and what unique visualization has been proposed?).
% evaluation & results
NAME is evaluated through xxx. (CASE study).
The results show that our system is capable of xxx.

%%%-----------------------------Contributions-------------------------------
To sum up, our key contributions are as follows:
\begin{itemize}
    \item
    A visual analytics system.
    
    \item
    ML space and raw data space -- xxx.
    
    \item
    Evaluation.
\end{itemize}

% Organization of the rest content
The description of how we organize the later sections.



%%% **************** Obsolete Versions **************** %%%

%%%----------------- Background: Interpretability & Transparency-----------------

%%% V2 by Furui
% To tackle these issues, researchers from diverse domains have made approaches by building ML models that are inherently interpretable ranging from decision tree~\cite{kho2012use} to deep sequential model with attention mechanism~\cite{choi2016retain}, or developing post-hoc explainability methods, 
% including feature attributions, rule surrogates~\cite{ming2018rulematrix}, case-based explanations, counterfactuals, and \etal.

%%% V1 by Dongyu:
% Despite the endeavour ML researchers have spent to improve model performance, the associated issues regarding transparency and interpretability that comes from real-world deployment process still remain remarkably challenging~\cite{sendak2020human}.
% In typical scenarios, ML models often only outputs one single value or classification, which makes clinicians difficult to understand why the model make a particular prediction and to handle any \mbox{potential disagreements}.
% As a result, ML-based prediction models yet have not been widely and reliably used in clinical decision support workflows ~\cite{jensen2012mining, miotto2016deep}.

% A successful clinical prediction models must consider both performance and interpretability. One common belief is that model performance has to be traded for the interpretability~\cite{choi2016retain}.
% To this end, interpretable models that supports rule finding (e.g., decision tree), similar case reasoning (e.g., K-Nearest Neighbors[cite]), and risk factors identifying (e.g., LASSO coefficients[cite]), are heavily used for clinical research with EHR data. In this work, we mainly consider another typical but more general type of approaches, using model-agnostic methods (e.g., Lime, Anchors, and Shap) to generate explanations. However, several unique challenges facing the introduction of such model-agnostic methods to clinicians are identified.


%%%----------------- Challenges ---------------------

%%% V3 - Dongyu
%However, ML-based prediction models yet have not been widely and reliably used in clinical decision support workflows ~\cite{jensen2012mining, miotto2016deep}. One of the key reasons would be that most existing XAI (eXplainable artificial intelligence) techniques generate explanations from the researchers' intuition of what constitutes a `good` explanation rather than stakeholders -- clinicians in this study~\cite{miller2019explanation, tonekaboni2019clinicians}.
%In the context of clinical practice, clinicians usually make decisions referring to \textbf{patients' original records}, like laboratory test reports, vital signs from a caring machine, and prescription list. Unfortunately, most existing XAI techniques are generating explanations based on \textbf{model input features} extracted from heterogeneous EHR data, such as the linear slope of the patient's systolic blood pressure in the last 24 hours \hl{[glyph]}. We found that explanations (\eg, feature importance) generated on feature space bring significant barriers for clinicians -- especially those with little data analysis experience -- to understand using their intuitions or domain experiences.

%%% V2 - Furui
% However, most existing techniques are criticized as ``building from data analysts' intuition but hard to understand by real end-users (\eg, clinicians)~\cite{miller2019explanation, tonekaboni2019clinicians}.'' In the context of clinical practice, this problem is even more severe because existing explanations are based on \textbf{model input features} extracted from heterogeneous EHR data (\eg, the linear slope of the patient's systolic blood pressure in the last 24 hours \hl{[glyph]}). Still, clinicians make decisions referring to \textbf{patients' original records}, like laboratory test reports, vital signs from a caring machine, and prescription list. The inconsistent data representations bring barriers for clinicians with little data analysis experience in understanding existing explanations especially when the explanations are made to numerous features extracted from diverse sources (e.g., symptoms, lab test, and prescriptions).


%%% V1 - Dongyu's draft on the relevant challenges
% First, EHR data is difficult to represent (i.e., featurize) and model, because of its multi-modality, high dimensionality, incompleteness, and systemmatic biases~\cite{miotto2016deep}. 
% Depending on the prediction task, one patient will be represented as a feature vector with each value representing a clinical feature coming from multiple sources such as \furui{demographics information (static feature), medications (multivariate events), and vital signs (time series such as pulse)}{static demographics information and statistical values of time series (e.g., mean value of the pulse in the last 6 hours.)}. 
% The performance of a prediction model is highly dependent on data representation and feature selection~\cite{bengio2013representation}.
% We argue that the interpretability of clinical features themselves is also one of the dominant features of a successful ML model, because the explanations (e.g., feature importance) generated by model-agnostic XAI methods are usually represented in the feature space instead of raw data space. Therefore, several questions come up: (1) what is the understandable features from the perspective of clinicians; (2) what is the good way of displaying the outputs of XAI methods to clinicians to facilitate their understanding.

% Second, clinicians are more familiar with EHR data in the raw format. Explanations in the raw data space is favored by clinicians and can provide more detailed information without introducing any ambiguity.
% So there is a desperate need to connect the explanations from the feature space to the raw data space, especially when a certain clinical feature is an aggregated feature (e.g., averaged heart rate).
% How to computationally convert and visually represent the explanations from feature space back to raw data space? 

% Third, most existing XAI work uses mainly the researchers' intuition of what constitutes a ``good`' explanation~\cite{miller2019explanation}.
% The same issue exists in the area of clinical research with EHR data.
% Current visual analytics tools\cite{ming2018rulematrix, kwon2018retainvis, jin2020carepre} appear to focus more on audience of ML experts or medical researchers with fairly sufficient data analysis background.
% In practice, clinicians' background may vary a lot and one may have little data analysis experience.
% In this regard, we have to keep away from using overly technical jargon or complicated visualizations. More importantly, the explaining workflow should be straightforward and easy to follow.



%%%-----------------Motivation: Research Goal & Scope-----------------------

%%% V1 - Furui
% This work aims to integrate existing post-hoc explainability methods into clinicians' decision workflow by bridging the feature-level explanations with patients' original records with interactive visualization. 
% The research scope is defined by 1) the ML model type, 2) the feature schema, and 3) the elementary explanations. 
% Specifically, we focus on classification models with tabular-style input features since they are among the most common practices in making clinical predictions.
% The features are generated through Featuretools\footnote{https://www.featuretools.com/}, an open-source framework for automated feature engineering from structured databases. (Algorithmic details are introduced in Section~\ref{sec:feature}.) \hl{[case]}
% We choose SHAP values as the elementary feature-level explanations because of their successful adaptations in explaining clinical prediction models.
% We attempt to address the following three research questions. First, what auxiliary information alongside ML predictions is needed to facilitate the clinicians' understanding in the results? Second, 
% As a summary, the goals of this work are studying (1) what auxiliary information alongside ML predictions is needed for clinicians; (2) what is the clinicians' favored explaining workflow when model-agnostics XAI techniques is integrated; and (3) and how a visualization solution can be built to display the auxiliary information and support such workflow?


%%% Furui;s notes: two reference articles motivate our work
% What Clinicians Want\cite{tonekaboni2019clinicians}: "To provide these explanations all clinicians ex- pressed the need to understand the clinically relevant model features that \textbf{align with current evidence-based medical practice}. The implemented system/model needs to provide clinicians with information about the context within which the model operates and promote awareness of situations where the model may fall short (e.g., model did not use specific history or did not have information around certain aspect of a patient)." (p5)

% Designing Theory-Driven User-Centric Explainable AI\cite{wang2019designing}: "Lack of Trust: Verify with Supplementary, Situational, Source Data. A lack of trust drove users to want to verify the AI’s decision by looking at raw data, in this case, patient case and physical exam notes, or recorded data, such as ECG readings, even if the AI model did not use such data. P7 felt that “without the context of the patient, [she] can’t diagnose based on the vitals itself. So [she] wouldn’t really trust”. In fact, this need to show raw situational data is commonly expected in different applications, such as showing test images in image recognition applications, and providing raw audio recordings in sound-based applications."
